Understanding the Effects of Permanent Faults in GPU's Parallelism Management and Control Units

Graphics Processing Units (GPUs) are over-stressed to accelerate High-Performance Computing applications and are used to accelerate Deep Neural Networks in several domains where they have a life expectancy of many years. These conditions expose the GPUs hardware to (premature) aging, causing permanent faults to arise after the usual end-of-manufacturing test. Techniques to assess the impact of permanent faults in GPUs are then strongly required, thus allowing to estimate the reliability risk and to possibly mitigate it. In this paper, we present a method to evaluate the effects of permanent faults affecting the GPU scheduler and control units, which are the most peculiar and stressed resources, along with the first figures that allow quantifying these effects. We characterize over 5.83x10^5 permanent fault effects in the scheduler and controllers of a gate-level GPU model. Then, we map the observed error categories in software by instrumenting the code of 13 applications and two convolutional neural networks, injecting more than 1.65x10^5 permanent errors. Our two-level fault injection strategy reduces the evaluation time from hundreds of years of gate-level evaluation to hundreds of hours.We found that faults in the GPU parallelism management units can modify the opcode, the addresses, and the status of thread(s) and warp(s). The large majority (up to 99%) of these hardware permanent errors impacts the running software execution. Errors affecting the instruction operation or resource management hang the code, while 45% of errors in the parallelism management or control-flow induce silent data corruptions.

==> src/error_model.tex <==
\section{RTL Reliability Evaluation}
\label{sec_error_model}

\begin{figure*}[t]%
   	\centering
    	\includegraphics[width=\textwidth]{Fig/AVF_P.pdf}
        \caption{AVF of the injections at RTL level on the functional units (FP32, INT, SFU), the scheduler, and pipeline registers for the different instructions. We plot the average AVF measured with the S, M, L input ranges.}
        \label{fig_AVF}
\end{figure*}

In this Section we detail the experimental results of the RTL characterization of faults effect in the considered GPU modules. We first describe the tested micro-benchmarks and mini-app, then we present the AVF and the fault syndrome description. % to be used in the software fault injection.

\subsection{Micro-benchmarks and mini-app description}
\label{sub_micro_description}
    %micro-benchmarks
    We design several micro-benchmarks to characterize the effects of RTL faults in integer, floating point, special functions, memory movements, and control-flow instructions. To observe the possible propagation of the single injected fault to individual or groups of threads, each micro-benchmark instantiates 64 threads (2 warps) executing the same instruction. We also test a mini-app (i.e., tile-based matrix multiplication) to better observer scheduler faults impact. It is worth noting that we inject only one fault in one targeted injection site per micro-benchmark execution. Possible multiple threads corruptions are caused by that single fault propagation and not by multiple fault injections.
    
    With the goal of characterizing the syndrome at the output of \textbf{arithmetic instructions} we have designed 8 specific CUDA micro-benchmarks to run on FlexGripPlus, one for each targeted floating point (FMUL, FADD, and FFMA), integer (IADD, IMUL, and IMAD), and special (FSIN, FEXP) instructions. Each of the 64 threads executes the same instruction without interactions between threads. We test the floating point and integer opcodes with three different pre-defined input ranges: \textit{Small} (S, both inputs in the range 6.8x10$^{-6}$ to 7.3x10$^{-6}$), \textit{Medium} (M, in the range 1.8 to 59.4), and \textit{Large} (L, in the range 3.8x10$^{9}$ to 12.5x10$^{9}$). {In the software fault injection any instruction with an input smaller than S (bigger than L) receives the S (L) syndrome, values in between receive the M syndrome. The range selection is heuristic, based on observed common values for SASS instructions inputs on the considered HPC and CNNs applications.}
    We also test a combinations of input ranges (first input S, second input L), obtaining very similar results than S and M ranges (not shown in the paper). For the special functions (FSIN, FEXP), we select three inputs according to the operational constraints in the SFU (in the range 0 to $\pi/2$), avoiding range reduction procedures. To avoid the bias of our results we perform a fault injection campaign on 4 different randomly selected values for each input range.
    % \todo{this also for FEXP?} ), yes the same HW block operates both functions.
    
    We also consider \textbf{memory movements} (GLD and GST) and \textbf{control-flow instructions} (BRA, ISET). The load and store micro-benchmark performs a load operation followed by a store operation. For the control-flow operation, we allocate a limited number of set-register instructions before the branch operation. A fault is detected when a set register is not correctly assigned or when the branch condition fails. We anticipate that, not surprisingly, in most cases faults in control-flow instructions collapse the execution leading to a DUE.
    
    %tiles
    Scheduler corruptions (and multiple threads corruptions in general) may have specific effects on the execution of codes in which threads interact with each other that may not be detected with the micro-benchmarks we have designed. As a specific and extremely important case study, we also characterize with RTL fault injection a \textbf{tile-based matrix multiplication (t-MxM)} mini-app. The choice of the mini-app is dictated by the observation that more than 70\% of operations inside a CNN is MxM related~\cite{yolov3}. To avoid memory latencies and, thus, improve matrix multiplication efficiency, large matrix multiplications are split into \textit{tiles} (smaller MxM). The tile size is set to maximize performances without saturating caches and registers. In our framework the optimal tile size is of 8x8. Each tile is assigned to a Streaming Multiprocessor and, then, all tiles are combined to form the output of MxM. In a CNN, the MxM output forms the layer output (feature map).
    
    To select the input for t-MxM, we execute LeNET and YOLOv3 with the MNIST~\cite{lenet1998} and VOC2012~\cite{yolov3} datasets, and observed that most tiles involved in convolution process have similar values, while the tiles at the edge of the feature map have a higher amount of zero operands, because of padding~\cite{yolov3, lenet1998}. We then characterize three inputs for the tiles with the RTL fault injection: (Max) Max tile (the tile with the highest sum of elements values), (Z) Zero tile (the tile with the highest number of zeros), and (R) Random tile (a tile selected among the ones without significantly biased values). We test 4 different values per tile type (Max, Z, R).
    %A preliminary sub-set of experiments allow us to analyze the fault effect on the output and also explore different input tile sizes. Firstly, the large number of layers and tiles-per-layer in a CNN makes unfeasible the execution of a complete fault injection campaign.
    

    
    %check this and justify with the previous sentence

\subsection{Architectural Vulnerability Factor}

    We perform fault injection in 6 GPU modules characterizing, for most modules, 12 SASS instructions and t-MxM, with different input sets (3 ranges and 4 values per range for arithmetic operations and t-MxM). In total, we perform 144 RTL fault-injection campaigns and, for each campaign, we inject more than 12,000 faults. That is, we present data from more than 1,72x10$^{6}$ fault injections. This guarantees a statistical margin error lower than 3\%.

%\subsection{Arithmetic Operations}
    %As introduced above, the arithmetic-type micro-benchmarks were evaluated in several modules of the GPU core. 

    
    
    %\todo{Esteban, what about adding a table with: OPCODE, description of the opcode, modules used, AVF for single thread, multiple thread, DUE?}
    
    % Not fully sure if useful, Fig 4 already present the same information., check sizes or style
   % \input{tables/table_modules_SDC_instructions}
    
    Figure \ref{fig_AVF} depicts, for injections in Functional Units (FP32, INT, SFU), Warp Scheduler, and Pipeline Registers, the AVF of each instruction. We have not considered injections in functional units for GLD, GST, BRA, and ISET as the FUs are idle when executing those instructions.
    In Figure~\ref{fig_AVF} we distinguish between SDCs affecting a single or multiple threads.
    As we have observed, {in accordance with}~\cite{Previlon2018}, that the AVF does not significantly depend on the input range (the AVF difference between S, M, and L inputs is always lower than 5\%), in Figure~\ref{fig_AVF} we show the average AVF measured with the three input ranges. %In Section~\ref{sub_syndrome} we show that the fault syndrome does depend on the input range.
    
    Figure~\ref{fig_AVF} shows that faults in the scheduler are less likely to impact the computation than faults in the functional units or pipeline (the y axes are on different scales). We recall that in our micro-benchmarks threads do not interact with each others, reducing the scheduling strain. In Section~\ref{sub_distribution} we show that the scheduler AVF increases significantly in more complex codes.
    Moreover, the functional units corruptions are much more likely to generate SDCs than DUEs while the outcome of injections in the pipeline is mainly dominated by DUEs. We further investigate the observed behaviours next.
    
    %SDCs
    More than 60\% of the SDCs caused by scheduler corruptions affect more than one thread for the INT and FP32 micro-benchmarks while injections in the functional units cause multiple threads corruption only for FSIN and FEXP. This is because the GPU has a dedicated ADD, MUL, and MAD unit for each thread while the few (two) available special function units (SFUs) need to be shared among different threads (see Figure~\ref{fig_scheme}). A deeper analysis of the multiple SDCs source revealed that the multiple corrupted threads observed with functional units corruptions in FSIN and FEXP are actually caused by faults in the control units of the SFUs. Interestingly, also pipeline injections cause multiple threads corruption. Investigating the causes for those multiple threads we found that, while most of pipeline registers ($\approx$84\%) store operands for each parallel core, there is also a small portion of registers ($\approx$16\%) devoted to control signals. The corruption of these latter registers caused the observed multiple threads SDCs.
    
    On the average, the number of corrupted parallel threads per warp is 1 for INT and FP32 functional units, 8 for the SFUs, 28 for the scheduler, and 18 for the pipeline. These averages show that the parallel operation's modules in the GPU, such as the scheduler and the pipeline, are more prone to corrupt a high number of multiple threads in a warp than others. %Faults in the INT and FP32 units only corrupted one thread. In contrast, the SFU units produced several corruptions mainly caused by the control structures and sharing registers described above. 
    A fault in the control structures and signals of the pipeline and, mainly, of the scheduler (which manages the warp operation), affects multiple threads. The lower number of threads corrupted in the pipeline is related to the number of available FUs and active threads at a given time (8 in our case). As some signals are not updated until a new warp is dispatched, their corruption affects, on the average, two of the four groups of 8 threads in a warp (32 threads).
    
    %DUEs
    The high DUE AVF for the pipeline (0.3\% for floating point, 2\% for integer, 4\% for special units, 10\% for control operations) is caused by corruptions of pipeline control registers that, despite being few ($\approx$16\%), are confirmed to be highly critical. The DUE AVF is exacerbated for special function units, because of the additional control signals required to share the use of the few available SFUs, and for control flow operations (GLD, GST, BRA, ISET) for which faults in the data path are likely to corrupt the control flow.
    
    The scheduler DUE AVF is almost constant (between 0.5\% and 0.6\%) for all instructions but BRA and ISET, for which the DUE AVF is about 0.8\%. Tracking the fault propagation we found that scheduler DUEs are caused by faults affecting structures in the controller devoted to store the state of the warp or memory addresses. In contrast, the scheduler SDCs are mostly caused by faults affecting warp state bits, so disabling active or enabling inactive threads. % in a warp. %Thus, the fault modifies the thread's flow and propagates the fault effect.
   
   % A similar analysis for memory operations (GLD and GST) show that both operations are specially sensitive to faults affecting structures (in the scheduler and in the pipeline registers) storing addresses to access memory resources, producing the observed SDCs (0.8\% and 2\%) in the scheduler and pipeline registers, respectively.
    
    %The AVF results in the control-flow micro-instructions (BRA and ISET) shows the high incidence of DUEs in the scheduler and the pipeline registers. In the scheduler's case, the percentage of DUE doubles the number of SDCs observed. The critical and sensitive operation of these instructions in the program-flow explains the high percentage of DUEs. 

%Esteban, I have commented this paragraph as we need space =)
  %  As observed in Figure~\ref{fig_AVF}, AVF seems to be independent for each micro-instructions. The pipeline includes control registers for each type of micro-instruction. Furthermore, each micro-instruction uses a certain number of submodules in a given structure, such as the functional units (i.e., the IADD instruction uses an adder instead of a multiplier in the INT FU), so several submodules may remain inactive. Moreover, control-flow micro-instructions are more prone to generate DUEs than SDCs as any effect on the program-flow might affect the entire micro-benchmark. %Other micro-instructions, such as those using the INT unit, produce more SDCs than DUEs by the minimum effect on the flow of the micro-benchmark. 

    %not clear to me
    
        %INT vs FLOAT vs FSIN FEXP vs control operation
    As observed in Figure~\ref{fig_AVF}, the functional units AVF for the floating point instructions (FADD, FMUL, FMAD) is much smaller than for the integer instructions (IADD, IMUL, IMAD). This is caused by the higher complexity and area of the floating point units, that are more than 3x larger than the integer units (see Table~\ref{tab:talbe_sizes_modules}). A larger area increases the number of injection sites, thus reducing the probability to hit a critical resource for computation. 
    
    \begin{figure}[t]%
   	\centering
   	\includegraphics[width=0.5\textwidth]{Fig/relative_ALL.pdf}
    \caption{Distribution of the fault syndrome (relative error) from the RTL fault injection in the Functional Units (top), Pipeline (middle), and Scheduler (bottom) for the floating point instructions executed with S, M, L inputs.}
    \label{fig_relative_FP}
\end{figure}
    
    
    It is worth noting that the AVF assumes that a fault has occurred and does not include any information about the probability for the fault to be generated. In order to consider also the fault generation probability, the modules AVF should be weighted with the module relative size (shown in Table~\ref{tab:talbe_sizes_modules}). A more accurate evaluation would consider the fault rate of the different modules, for which either proprietary information on the technology sensitivity or beam experiments would be necessary. As a first evaluation, combining Table~\ref{tab:talbe_sizes_modules} and Figure~\ref{fig_AVF}, we can say that functional units, having a huge size and high AVF, are likely to be the source of most SDCs, while pipelines are likely to be the cause of most DUEs.
    
%     \todo{the weighted AVF can be removed if space is needed.}
%     The \textit{weighted AVF} is calculated according to Eq.~\ref{eq_norm}:
    
%     \begin{equation}
%     WeightedAVF_{module} = AVF_{module}\times{\frac{size\ module} {total\ size}}
%     \label{eq_norm}
%     \end{equation}
    
%     The weighted AVF gives an idea of the probability for the fault to occur in a module (proportional to its size, as shown in Table~\ref{table of sizes/description}) together with the probability for the fault in the module to propagate affecting the micro-instruction execution. Please notice that the weighted AVF is not intended to precisely compare the sensitivity or error rate of the different modules, for which either proprietary information on the technology sensitivity or beam experiments would be necessary.
    
%     Figure~\ref{fig_norm_AVF} shows the \textit{weighted} AVF, combining SDCs (single and multiple threads) and DUEs, for the considered modules and micro-instructions. Functional units are, by far, the more likely to induce errors in the arithmetic instructions output (and have no impact on control instructions that do not use FUs). This results from the combination of high AVF (Fig~\ref{fig_AVF}) and large area (see Table~\ref{table of sizes/description}). Pipeline faults have a significant impact in the execution of control instructions, because of the high amount of DUEs and are much less critical for the execution of arithmetic operations. Finally, the scheduler is the less likely source of errors in all tested benchmarks. As already mentioned, this is also due to the simple structure of the micro-benchmark. The analysis of t-MxM in Section~\ref{sub_distribution} shows that the scheduler impact is exacerbated when more complex codes are executed.
    
%     %A detailed analysis reveals that almost 95\% of the fault effects were caused by faults affecting the control registers in the evaluated structure, so explaining the observed behavior. For both modules (Scheduler and Pipeline registers) the corruption of the outputs are caused in locations devoted to control the program operation and to manage the thread-flow. An equivalent behavior is observed for the FSIN and FEXP micro-benchmarks. 
    
    
    
    
%     %The results show the reliability impact of each analyzed instruction when affected by faults in a targeted modules.
%   %In the one hand, the fault sensibility in the scheduler module remains almost constant when changing input patterns for each micro-benchmark. A similar behavior is observed for the pipeline registers, which in principle are registers storing mostly operands for each parallel core \color{red}(2/3)\color{black}, but it is also composed with a small portion of register devoted to control signals \color{red}(1/3)\color{black}. 
    
    
    
%     %On the other hand, the corruption effect caused by faults in the execution units varies across the micro-benchmarks and the input patterns. In most cases, parts of the execution cores are active depending on the input pattern.

%     % Regarding the ranges of the fault model for each arithmetic instruction, Figure \ref{fig_AVF2} represent the distribution of the relative error obtained after comparing the golden values and the corrupted outputs. An additional analysis of binary distribution was performed. However, clear patterns for the execution units were not feasible to find.
%     % \color{blue}
% %1 - arithmetic operations, inputs, AVF, relative error
% %\color{black}


%     \begin{figure}[t]%
%     	\centering
%     	\includegraphics[width=0.485\textwidth]{Fig/AVF_normalized_P.pdf}
%         \caption{Weighted total AVF (SDC and DUE) for the micro-instructions. The AVF of each module has been weighted to the relative module size (Eq.~\ref{eq_norm}).}
%         \label{fig_norm_AVF}
%     \end{figure}

    % \begin{figure}[t]%
    % 	\centering
    % 	\includegraphics[width=0.485\textwidth]{Fig/scheduler.png}
    %     \caption{Draft of the AVF in the Scheduler. }
    %     \label{fig_AVF1}
    % \end{figure}

    % \begin{figure}[t]%
    % 	\centering
    % 	\includegraphics[width=0.485\textwidth]{Fig/dummy_figure.png}
    %     \caption{Draft of the Relative error.}
    %     \label{fig_AVF2}
    % \end{figure}


    % \begin{figure}[t]%
    % 	\centering
    % 	\includegraphics[width=0.485\textwidth]{Fig/execution_units.png}
    %     \caption{Draft of the AVF in each execution unit. }
    %     \label{fig_AVF3}
    % \end{figure}

    % \begin{figure}[t]%
    % 	\centering
    % 	\includegraphics[width=0.485\textwidth]{Fig/pipes.png}
    %     \caption{Draft of the AVF in the pipeline registers. }
    %     \label{fig_AVF4}
    % \end{figure}

    % \begin{figure*}[t]%
    % 	\centering
    % 	\includegraphics[width=\textwidth]{Fig/AVF_normalized.png}
    %     \caption{Updated draft of the relative normalized AVF. 
    %     determined as the individual AVF module size/accumulated size evaluated modules }
    %     \label{fig_scheme}
    % \end{figure*}





%\subsection{Control-flow and Memory-type Operations}





%\color{red}
%\subsection{Study Case Application (Matrix multiplication)}


\subsection{Fault Syndrome}
\label{sub_syndrome}

For each SDC observed at the instructions output we keep a \textit{detailed report} (described in Section~\ref{sec_rtl_fi}), that includes also the corrupted output value. We characterize the fault syndrome by measuring the \textit{relative error} induced by the fault. We also perform an additional analysis of the binary distribution of errors at the output (how many bits of the output are corrupted and in which position). Nevertheless, there was not a clear pattern for the bits corruption (in the large majority of cases, $\approx$24 bits are wrong, randomly distributed). This is in accordance with the fact that computational faults induce a not-obvious syndrome, as also observed in~\cite{Subasi2018}.

The relative error syndrome analysis highlights a very interesting trend. Figures~\ref{fig_relative_FP} and~\ref{fig_relative_INT} show the distribution of relative errors for the tested micro-benchmarks. We plot, in the y-axes, the percentage of observed SDCs that modify the instruction output value from less than $10^{-8}$ to over $10^{2}$. That is, 0.2\% of SDCs observed on FADD executed with the Small input range modify the output value by $10^{-6}\times$ and 0.3\% of SDCs observed on FFMA executed with the Large input range modify the output value by $10\times$.

    \begin{figure}[t]%
   	\centering
   	\includegraphics[width=0.5\textwidth]{Fig/relative_ALL_INT.pdf}
    \caption{Distribution of the fault syndrome (relative error) from the RTL fault injection in the Functional Units (top), Pipeline (middle), and Scheduler (bottom) for the integer instructions executed with S, M, L inputs.} % Some configurations overlap.}
    \label{fig_relative_INT}
\end{figure}

As depicted in Figures~\ref{fig_relative_FP} for floating point and in Figure~\ref{fig_relative_INT} for integer instructions, the relative difference between the observed corrupted values and the expected value does not follow a Gaussian distribution. For all instructions there is a clear peak that depends on the input range and on the injection site. In some configurations (FFMA and FMUL FU injections with L input) two peaks are present. It is also interesting to notice that the relative difference distribution is narrow, if compared to the floating point or integer representation range. Only in few cases (less than 0.05\%), we observed a syndrome with a relative error higher than $10^2$ (i.e., the corrupted output value is 100x bigger/smaller than the expected one). This observation attests that even injecting a random number of bit-flips in the instruction output might not be realistic. Our results show that there is a limited difference between corrupted and correct values. {Interestingly, the median of the syndrome values between S/M/L varies by just $\sim$1\% in all cases but MUL and FMA, for which the median changes by up to 30\% (bigger input range has higher median). Only for MUL and FMA, then, we expect a syndrome dependence on the input.}

Once the opcode, the input range, and the injection site have been determined, to injecting the syndrome in software we need to select a relative error, statistically taken from the data presented in Figures~\ref{fig_relative_FP} and~\ref{fig_relative_INT} and available in~\cite{REPO}. The syndrome (as relative error) {does not follow a Gaussian distribution (all distributions have a p-value smaller than 0.05 on the Shapiro-Wilk test)}, but rather follows a \textit{power law} distribution~\cite{clauset2007}, in which few events are predominant.
We create a Pseudo-Random Number Generator (PRNG) function, based on the mathematical formalization in~\cite{clauset2007}, that generates the syndrome to be injected as follows:
\begin{equation}
relative\_error = P^{-1}(1 - r) = x_{min}(1 - r)^{-1/(\alpha - 1)}
\label{eq_power}
\end{equation}

{Where $0 \leq r < 1$ is a uniformly distributed random value, %In this work, we use the random float uniform distributed generator available on the C++ standard library.  
$\alpha$ is the scaling factor, and $x_{min}$ is the values lower bound. Both parameters are extracted from our data based on the methods described in}~\cite{clauset2007}.

% https://stats.stackexchange.com/a/406705
% E exatamente o que esta na resposta xmin e o limite superior da distribuicao da figura 6 e 7
% alpha e o scaling factor da distribuicao na figura 6 e 7
% r vem da fucao random do C++

%\todo{Fernando, acho que seria melhor definir os parametros usando a terminologia e os valores do nosso paper. Nao sei exactamente o que sao essas variaeis.} 


%binary distribution inconclusive (pseudo random)

    
\subsection{Tiled MxM errors distribution}
\label{sub_distribution}



\begin{figure}[t]%
  	\centering
  	\includegraphics[width=0.34\textwidth]{Fig/AVF_tiles.pdf}
\caption{AVF of the scheduler (left) and pipeline (right) for DUEs, single and multiple thread SDCs for the Max, Zero, and Random t-MxM.}
\label{fig_mxm_avf}
\end{figure}


\begin{figure}[t]%
  	\centering
  	\includegraphics[width=0.485\textwidth]{Fig/fig7.png}
\caption{Spatial distribution of the multiple corrupted elements patterns observed in the RTL injection on the mini-app t-MxM. Arrows indicate that neither the position of the observed pattern nor the block size are fixed.}
\label{fig_mxm_spatial}
\end{figure}


    
    
    % Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Distribution of the multiple patterns (single corrupted elements are not listed) observed with t-MxM.}
\label{tab:mxm}
\begin{tabular}{l|l|l|l|l|l|l}
\textbf{inj. site} & \textbf{row}  & \textbf{col.} & \textbf{row+col.} & \textbf{block} & \textbf{rand.}  & \textbf{all} \\ \hline
 scheduler & 0.96\%  & 0.07\%  & 0.45\% & 5.77\% & 0.69\%  & 54.6\% \\ \hline
 pipeline &  45.4\% & 1.36\% & 1.04\%  & 7.29\% & 0.42\% & 4.17\% \\ \hline
%\textbf{injection site} & \textbf{block} & \textbf{random}  & \textbf{(almost) all}  \\ \hline
% scheduler & 5.77\% & 0.69\%  & 54.6\%  \\ \hline
%pipeline & 7.29\% & 0.42\% & 4.17\% \\ \hline
\end{tabular}
\end{table}


To better study the impact of multiple threads corruptions in codes with threads interactions we have characterized, with the RTL fault injector, the mini-app t-MxM. We test three input types (Max, Zero, and Random tiles), averaging the results obtained with four values per each input type. For t-MxM, we inject faults in the scheduler and pipeline registers but not in the functional units. Faults in this latter module, as shown in Figure~\ref{fig_AVF}, would not cause multiple threads corruptions in t-MxM (there is no transcendental operation). The effects of the single thread SDC would then be the same as the ones observed injecting the FU syndrome in software, without requiring a costly RTL injection. 

Figure~\ref{fig_mxm_avf} shows the average AVF for DUEs, single and multiple corrupted elements in the t-MxM output for injections in the scheduler and pipeline. We recall that we inject one fault per execution: the multiple corrupted elements are caused by the single fault propagation.

A major difference from the micro-benchmarks AVF in Figure~\ref{fig_AVF} is that, for t-MxM, the scheduler AVF is higher than the pipeline one. As mentioned, while the micro-benchmarks are very simple and do not implement threads interactions, t-MxM also includes several instructions for computing memory addresses and threads indices. The higher strain on the scheduler and the higher portion of time spent in scheduling operation increases the AVF (for both SDCs and DUEs). On the contrary, the pipeline AVF is higher in the micro-benchmarks because, when a fault appears at the first instruction output, it is marked as SDCs, without further chances to be masked (there is no other computation). In t-MxM an instruction's wrong output can be masked in a downstream operation (for instance, with a multiplication by zero). This statement is supported by our pipeline data in Figure~\ref{fig_mxm_avf}, that shows a much lower SDC AVF for the Z tile.

An additional interesting result from Figure~\ref{fig_mxm_avf} is that the portion of SDCs that affect multiple elements is very high (at least 70\% of scheduler induced and 50\% of pipeline induced SDCs).
We can further study the multiple errors at the t-MxM output by visualizing the geometrical distribution of the corrupted elements. In Figure~\ref{fig_mxm_spatial} we plot the 6 different spatial multiple corrupted elements distribution patterns that we have observed injecting faults in the scheduler and pipeline registers. We have observed corrupted elements distributed in a row, a column, a row and a column, a block of elements (varying in size), randomly, and all (or almost all) elements corrupted.
Table~\ref{tab:mxm} lists the percentage of occurrences of the different patterns (single SDCs are not listed). As the distribution of the observed patterns is very similar in the three inputs we test (M, Z, R tiles), we list the average distributions.

Interestingly, pipeline injection mostly produces corrupted rows, while scheduler injection is more likely to affect the whole output matrix. Having a whole column corrupted is very unlikely, for both injection sites. This is because t-MxM calculation is row-major and, as mentioned, the distribution of these error patterns depends not only on the way the GPU hardware reacts to the faults, but also on the software propagation. While this multiple elements distribution is not generic, the choice of t-MxM extended evaluation is dictated by its importance in CNNs execution. As shown in~\cite{tr2019, Ibrahim2020}, the observed multiple errors patterns (but not single element corruptions) can indeed induce misdetections in CNNs.

%while it is highly unlikely for single errors to induce , .

We have also characterized the syndrome of t-MxM. Most of the syndromes are concentrated in few values, again following a power-law distribution. In Figure~\ref{fig_mxm_spatial_3d} we plot the relative error distribution for two examples: a row and a block error. As shown, the relative error distribution varies among the corrupted elements. To inject the t-MxM syndrome in software, then, we use Equation~\ref{eq_power} to select the range of the relative errors for all the elements to corrupt. In this range, we again select a power law distribution for the corruption of the individual output elements.

\begin{figure}[t]%
  	\centering
  	\includegraphics[width=0.49\textwidth]{Fig/3D.pdf}
\caption{Variance distribution of relative errors for an example of Row (left) and Block (Right) patterns with multiple corrupted elements.}
\label{fig_mxm_spatial_3d}
\end{figure}






==> tables/table_avf_units.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{lscape}
\begin{landscape}
\begin{table}[]

\caption{AVF per error on the analyzed units}
\label{tab:table_modules_SDC}
\centering

\resizebox{0.48\textwidth}{!}{%


\begin{tabular}{ccccccc}
\hline
\textbf{Unit}                                   & \textbf{\begin{tabular}[c]{@{}c@{}}Total HW faults \\ per unit\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hang faults \\ (HW)\end{tabular}} & \textbf{Error} & \textbf{\begin{tabular}[c]{@{}c@{}}HW Faults causing \\ the error\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}AVF \\ (per error)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Times an error\\  was produced (SW)\end{tabular}} \\ \hline
\multirow{8}{*}{\textit{\textbf{WSC}}}          & \multirow{8}{*}{29,850}                                                      & \multirow{8}{*}{1069}                                                & IAC            & 310                                                                             & 1.08                                                                & 566                                                                                  \\
                                                &                                                                              &                                                                      & IAL            & 2,089                                                                           & 7.26                                                                & 5,233                                                                                \\
                                                &                                                                              &                                                                      & IAT            & 1,288                                                                           & 4.48                                                                & 4,662                                                                                \\
                                                &                                                                              &                                                                      & IAW            & 2,168                                                                           & 7.53                                                                & 5,493                                                                                \\
                                                &                                                                              &                                                                      & IOC            & 1,521                                                                           & 5.28                                                                & 5,599                                                                                \\
                                                &                                                                              &                                                                      & IPP            & 916                                                                             & 3.18                                                                & 5,579                                                                                \\
                                                &                                                                              &                                                                      & IRA            & 2,605                                                                           & 9.05                                                                & 9,659                                                                                \\ \cline{4-7} 
                                                &                                                                              &                                                                      & \textbf{Total} & \textbf{10,897}                                                                 & \textbf{37.86}                                                      & \textbf{36,791}                                                                      \\ \hline
\multirow{9}{*}{\textit{\textbf{Fetch unit}}}   & \multirow{9}{*}{9,320}                                                       & \multirow{9}{*}{108}                                                 & IAC            & 44                                                                              & 0.48                                                                & 216                                                                                  \\
                                                &                                                                              &                                                                      & IAL            & 153                                                                             & 1.66                                                                & 314                                                                                  \\
                                                &                                                                              &                                                                      & IAT            & 720                                                                             & 7.82                                                                & 3,901                                                                                \\
                                                &                                                                              &                                                                      & IAW            & 256                                                                             & 2.78                                                                & 607                                                                                  \\
                                                &                                                                              &                                                                      & IOC            & 1,413                                                                           & 15.34                                                               & 12,794                                                                               \\
                                                &                                                                              &                                                                      & IPP            & 98                                                                              & 1.06                                                                & 714                                                                                  \\
                                                &                                                                              &                                                                      & IRA            & 451                                                                             & 4.9                                                                 & 1,665                                                                                \\
                                                &                                                                              &                                                                      & IVOC           & 1,356                                                                           & 14.72                                                               & 8,880                                                                                \\ \cline{4-7} 
                                                &                                                                              &                                                                      & \textbf{Total} & \textbf{4,491}                                                                  & \textbf{48.75}                                                      & \textbf{29,091}                                                                      \\ \hline
\multirow{12}{*}{\textit{\textbf{Decode unit}}} & \multirow{12}{*}{10,874}                                                     & \multirow{12}{*}{269}                                                & WV             & 439                                                                             & 4.14                                                                & 702                                                                                  \\
                                                &                                                                              &                                                                      & IAC            & 54                                                                              & 0.51                                                                & 187                                                                                  \\
                                                &                                                                              &                                                                      & IAL            & 126                                                                             & 1.19                                                                & 245                                                                                  \\
                                                &                                                                              &                                                                      & IAT            & 929                                                                             & 8.76                                                                & 3,410                                                                                \\
                                                &                                                                              &                                                                      & IIO            & 1,053                                                                           & 9.93                                                                & 2,524                                                                                \\
                                                &                                                                              &                                                                      & IMD            & 1,775                                                                           & 16.74                                                               & 6,817                                                                                \\
                                                &                                                                              &                                                                      & IMS            & 1,943                                                                           & 18.32                                                               & 14,776                                                                               \\
                                                &                                                                              &                                                                      & IOC            & 1,210                                                                           & 11.41                                                               & 3,416                                                                                \\
                                                &                                                                              &                                                                      & IPP            & 292                                                                             & 2.75                                                                & 1,194                                                                                \\
                                                &                                                                              &                                                                      & IRA            & 332                                                                             & 3.13                                                                & 765                                                                                  \\
                                                &                                                                              &                                                                      & IR             & 1,982                                                                           & 18.69                                                               & 9,158                                                                                \\ \cline{4-7} 
                                                &                                                                              &                                                                      & \textbf{Total} & \textbf{10,135}                                                                 & \textbf{95.57}                                                      & \textbf{43,194}                                                                      \\ \hline
\end{tabular}
}
\end{table}
\end{landscape}








==> tables/table_sizes_modules.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}

% \begin{table}[]
% \caption{Evaluated modules, sizes and instructions used per module}
% \label{tab:talbe_sizes_modules}

% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{cccc}
% \hline
% Module                                                    & RTL Size (Flip-Flops) & Type           & Instructions     \\ \hline
% FP32                                                      & 4451                  & Execution/Data & FADD, FMUL, FFMA \\ \hline
% INT                                                       & 1542                  & Execution/Data & IADD, IMUL, IMAD \\ \hline
% SFU                                                       & 3231                  & Execution/Data & FSIN, FEXP       \\ \hline
% \begin{tabular}[c]{@{}c@{}}SFU \\ controller\end{tabular} & 190                   & Control        & FSIN, FEXP       \\ \hline
% \begin{tabular}[c]{@{}c@{}}Scheduler \\ controller\end{tabular} &
%   3358 &
%   Control &
%   \begin{tabular}[c]{@{}c@{}} FADD, FMUL, FFMA, \\ IADD, IMUL, IMAD, \\ FSIN, FEXP, GLD,\\  GST, BRA, ISET\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Pipeline \\ Registers\end{tabular} &
%   10949 &
%   Control/Data &
%   \begin{tabular}[c]{@{}c@{}}FADD, FMUL, FFMA,\\ IADD, IMUL, IMAD, \\ FSIN, FEXP, GLD,\\ GST. BRA, ISET\end{tabular} \\ \hline
% \end{tabular}%
% }
% \end{table}

\begin{table}[]
\caption{Evaluated modules, sizes and instructions used per module}
\label{tab:talbe_sizes_modules}

\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{cccc}
\hline
Module                                                    & RTL Size (Flip-Flops) & Type           & Instructions     \\ \hline
FP32                                                      & 4,451                  & Execution/Data & FADD, FMUL, FFMA \\ \hline
INT                                                       & 1,542                  & Execution/Data & IADD, IMUL, IMAD \\ \hline
SFU                                                       & 3,231                  & Execution/Data & FSIN, FEXP       \\ \hline
\begin{tabular}[c]{@{}c@{}}SFU controller\end{tabular} & 190                   & Control        & FSIN, FEXP       \\ \hline
\begin{tabular}[c]{@{}c@{}}Scheduler controller\end{tabular} &
  3,358 &
  Control &
  \begin{tabular}[c]{@{}c@{}} ALL\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Pipeline Registers\end{tabular} &
  10,949 &
  Control/Data &
  \begin{tabular}[c]{@{}c@{}}ALL\end{tabular} \\ \hline
\end{tabular}%
}
\end{table}
